Temporal stability in human interaction networks

This paper reports on stable (or invariant) properties of human interaction networks, with benchmarks derived from public email lists. Activity, recognized through messages sent, along time and topology were observed in snapshots in a timeline, and at different scales. Our analysis shows that activity is practically the same for all networks across timescales ranging from seconds to months. The principal components of the participants in the topological metrics space remain practically unchanged as different sets of messages are considered. The activity of participants follows the expected scale-free trace, thus yielding the hub, intermediary and peripheral classes of vertices by comparison against the Erd\"os-R\'enyi model. The relative sizes of these three sectors are essentially the same for all email lists and the same along time. Typically, $<15\%$ of the vertices are hubs, 15-45\% are intermediary and $>45\%$ are peripheral vertices. Similar results for the distribution of participants in the three sectors and for the relative importance of the topological metrics were obtained for 12 additional networks from Facebook, Twitter and ParticipaBR. These properties are consistent with the literature and may be general for human interaction networks, which has important implications for establishing a typology of participants based on quantitative criteria.

==> tables/tab1Geral.tex <==
LAU & 2003-06-29  & 2005-07-23  & 1181  & 3372  & 5 \\\hline
LAD & 2003-06-30  & 2009-10-07  & 1268  & 3109  & 4 \\\hline
MET & 2005-08-01  & 2008-03-07  & 492  & 4607  & 23 \\\hline
CPP & 2002-03-12  & 2009-08-25  & 1052  & 4506  & 7 \\\hline


==> tables/tab2TimeCPP.tex <==
seconds & --//--  & 3.31  & 1.00  & 28205.46  & 0.79  & 0.78  & 0.03 \\\hline
minutes & --//--  & 3.18  & 0.99  & 12275.59  & 0.79  & 0.78  & 0.03 \\\hline
hours & -9.39  & 1.48  & 0.67  & 3.91  & 0.09  & 0.87  & 0.02 \\\hline
weekdays & -0.17  & 1.83  & 0.81  & 12.66  & 0.39  & 0.95  & 0.01 \\\hline
month days & -10.12  & 3.16  & 0.99  & 10789.17  & 0.65  & 0.85  & 0.02 \\\hline
months & 0.15  & 2.34  & 0.93  & 115.49  & 0.67  & 0.92  & 0.02 \\\hline


==> tables/tab2TimeLAD.tex <==
seconds & --//--  & 3.13  & 0.99  & 9070.17  & 0.78  & 0.78  & 0.03 \\\hline
minutes & --//--  & 3.60  & 1.00  & 205489.40  & 0.82  & 0.78  & 0.03 \\\hline
hours & -9.61  & 1.52  & 0.68  & 4.36  & 0.10  & 0.87  & 0.02 \\\hline
weekdays & -0.03  & 2.03  & 0.87  & 29.28  & 0.58  & 0.95  & 0.01 \\\hline
month days & -2.65  & 2.93  & 0.99  & 2657.77  & 0.67  & 0.85  & 0.02 \\\hline
months & -0.56  & 2.14  & 0.90  & 44.00  & 0.44  & 0.92  & 0.02 \\\hline


==> tables/tab2TimeLAD__.tex <==
seconds & --//--  & 3.13  & 0.99  & 9070.17    \\\hline
minutes & --//--  & 3.60  & 1.00  & 205489.40  \\\hline
hours & -9.61  & 1.52  & 0.68  & 4.36          \\\hline
weekdays & -0.03  & 2.03  & 0.87  & 29.28      \\\hline
month days & -0.07  & 2.94  & 0.99  & 2754.16  \\\hline
months & -0.56  & 2.14  & 0.90  & 44.00        \\\hline


==> tables/tab2TimeLAU.tex <==
seconds & --//--  & 3.31  & 1.00  & 29337.65  & 0.78  & 0.78  & 0.03 \\\hline
minutes & --//--  & 3.13  & 0.99  & 8879.19  & 0.76  & 0.78  & 0.03 \\\hline
hours & -8.76  & 1.56  & 0.71  & 4.92  & 0.12  & 0.87  & 0.02 \\\hline
weekdays & -0.21  & 2.14  & 0.90  & 45.41  & 0.62  & 0.95  & 0.01 \\\hline
month days & -0.64  & 2.76  & 0.98  & 1001.75  & 0.67  & 0.85  & 0.02 \\\hline
months & 3.55  & 2.30  & 0.93  & 94.53  & 0.64  & 0.92  & 0.02 \\\hline


==> tables/tab2TimeMET.tex <==
seconds & --//--  & 3.06  & 0.99  & 5910.47  & 0.79  & 0.77  & 0.03 \\\hline
minutes & --//--  & 3.14  & 0.99  & 9696.29  & 0.75  & 0.77  & 0.03 \\\hline
hours & -9.20  & 1.35  & 0.60  & 2.76  & 0.05  & 0.87  & 0.02 \\\hline
weekdays & -0.27  & 1.86  & 0.82  & 13.82  & 0.35  & 0.95  & 0.02 \\\hline
month days & 3.58  & 2.49  & 0.95  & 237.30  & 0.64  & 0.85  & 0.02 \\\hline
months & -2.92  & 1.73  & 0.78  & 9.20  & 0.33  & 0.92  & 0.02 \\\hline


==> tables/tabExtra.tex <==
F1 & Facebook  & friendship  & no  & the friendship network of Renato Fabbri (author)  & 1367  & 28606 \\\hline
F2 & Facebook  & friendship  & no  & the friendship network of Massimo Canevacci (senior anthropologist)  & 4764  & 59995 \\\hline
F3 & Facebook  & friendship  & no  & the friendship network of a brazilian direct democracy group  & 3599  & 59471 \\\hline
F4 & Facebook  & friendship  & no  & the friendship network of the Silicon Valley Global Network group  & 2026  & 15586 \\\hline
F5 & Participa.br  & friendship  & no  & the friendship network of a brazilian federal social participation portal  & 443  & 910 \\\hline
I1 & Facebook  & interaction  & yes  & the interaction network of the Silicon Valley Global Network group  & 104  & 154 \\\hline
I2 & Facebook  & interaction  & yes  & the interaction network of a Solidarity Economy group  & 64  & 120 \\\hline
I3 & Facebook  & interaction  & yes  & the interaction network of a brazilian direct democracy group  & 214  & 310 \\\hline
I4 & Facebook  & interaction  & yes  & the interaction network of the 'Cience with Frontiers' group  & 530  & 1658 \\\hline
I5 & Participa.br  & interaction  & yes  & the interaction network of a brazilian federal social participation portal  & 222  & 300 \\\hline
TT1 & Twitter  & retweet  & yes  & the retweet network of $\approx 22k$ tweets with the hashtag \#arenaNETmundial  & 2772  & 7222 \\\hline
TT2 & Twitter  & retweet  & yes  & same as TT1, but disconnected agents are not discarded  & 2975  & 7222 \\\hline


==> tables/tabHoursALL.tex <==
\begin{center}
\begin{tabular}{l || c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |}\hline
 & \multicolumn{4}{c|}{LAU} & \multicolumn{4}{c|}{LAD} & \multicolumn{4}{c|}{MET} & \multicolumn{4}{c|}{CPP} \\\hline
 & 1h & 4h & 6h & 12h & 1h & 4h & 6h & 12h & 1h & 4h & 6h & 12h & 1h & 4h & 6h & 12h \\\hline
0h & \multirow{1}{*}{ 3.58 }  & \multirow{4}{*}{ 8.49 }  & \multirow{6}{*}{ 10.14 }  & \multirow{12}{*}{ 36.88 }  & \multirow{1}{*}{ 4.01 }  & \multirow{4}{*}{ 9.37 }  & \multirow{6}{*}{ 10.78 }  & \multirow{12}{*}{ 33.11 }  & \multirow{1}{*}{ 2.87 }  & \multirow{4}{*}{ 6.31 }  & \multirow{6}{*}{ 7.15 }  & \multirow{12}{*}{ 29.33 }  & \multirow{1}{*}{ 3.66 }  & \multirow{4}{*}{ 9.30 }  & \multirow{6}{*}{ 10.67 }  & \multirow{12}{*}{ 33.76 }  \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}
1h & \multirow{1}{*}{ 2.22 }  & & & & \multirow{1}{*}{ 2.52 }  & & & & \multirow{1}{*}{ 1.77 }  & & & & \multirow{1}{*}{ 2.76 }  & & & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}
2h & \multirow{1}{*}{ 1.63 }  & & & & \multirow{1}{*}{ 1.79 }  & & & & \multirow{1}{*}{ 1.04 }  & & & & \multirow{1}{*}{ 1.79 }  & & & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}
3h & \multirow{1}{*}{ 1.06 }  & & & & \multirow{1}{*}{ 1.06 }  & & & & \multirow{1}{*}{ 0.64 }  & & & & \multirow{1}{*}{ 1.10 }  & & & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
4h & \multirow{1}{*}{ 0.84 }  & \multirow{4}{*}{ 5.20 }  & & & \multirow{1}{*}{ 0.75 }  & \multirow{4}{*}{ 3.81 }  & & & \multirow{1}{*}{ 0.47 }  & \multirow{4}{*}{ 2.89 }  & & & \multirow{1}{*}{ 0.68 }  & \multirow{4}{*}{ 3.44 }  & & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}
5h & \multirow{1}{*}{ 0.82 }  & & & & \multirow{1}{*}{ 0.66 }  & & & & \multirow{1}{*}{ 0.38 }  & & & & \multirow{1}{*}{ 0.69 }  & & & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}\cline{3-3}\cline{7-7}\cline{11-11}\cline{15-15}
6h & \multirow{1}{*}{ 1.17 }  & & \multirow{6}{*}{ 26.74 }  & & \multirow{1}{*}{ 0.85 }  & & \multirow{6}{*}{ 22.33 }  & & \multirow{1}{*}{ 0.72 }  & & \multirow{6}{*}{ 22.18 }  & & \multirow{1}{*}{ 0.83 }  & & \multirow{6}{*}{ 23.09 }  & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}
7h & \multirow{1}{*}{ 2.37 }  & & & & \multirow{1}{*}{ 1.56 }  & & & & \multirow{1}{*}{ 1.33 }  & & & & \multirow{1}{*}{ 1.24 }  & & & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
8h & \multirow{1}{*}{ 3.53 }  & \multirow{4}{*}{ 23.20 }  & & & \multirow{1}{*}{ 2.95 }  & \multirow{4}{*}{ 19.93 }  & & & \multirow{1}{*}{ 2.67 }  & \multirow{4}{*}{ 20.14 }  & & & \multirow{1}{*}{ 2.28 }  & \multirow{4}{*}{ 21.03 }  & & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}
9h & \multirow{1}{*}{ 6.04 }  & & & & \multirow{1}{*}{ 4.66 }  & & & & \multirow{1}{*}{ 4.40 }  & & & & \multirow{1}{*}{ 4.52 }  & & & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}
10h & \multirow{1}{*}{ 6.83 }  & & & & \multirow{1}{*}{ 5.92 }  & & & & \multirow{1}{*}{ 6.29 }  & & & & \multirow{1}{*}{ 6.62 }  & & & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}
11h & \multirow{1}{*}{ 6.79 }  & & & & \multirow{1}{*}{ 6.40 }  & & & & \multirow{1}{*}{ 6.78 }  & & & & \multirow{1}{*}{ 7.61 }  & & & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}\cline{3-3}\cline{7-7}\cline{11-11}\cline{15-15}\cline{4-4}\cline{8-8}\cline{12-12}\cline{16-16}
12h & \multirow{1}{*}{ 6.11 }  & \multirow{4}{*}{ 24.68 }  & \multirow{6}{*}{ 35.66 }  & \multirow{12}{*}{ 63.12 }  & \multirow{1}{*}{ 6.41 }  & \multirow{4}{*}{ 24.82 }  & \multirow{6}{*}{ 37.24 }  & \multirow{12}{*}{ 66.89 }  & \multirow{1}{*}{ 7.33 }  & \multirow{4}{*}{ 28.65 }  & \multirow{6}{*}{ 42.22 }  & \multirow{12}{*}{ 70.67 }  & \multirow{1}{*}{ 6.44 }  & \multirow{4}{*}{ 25.05 }  & \multirow{6}{*}{ 37.63 }  & \multirow{12}{*}{ 66.24 }  \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}
13h & \multirow{1}{*}{ 6.26 }  & & & & \multirow{1}{*}{ 6.12 }  & & & & \multirow{1}{*}{ 7.08 }  & & & & \multirow{1}{*}{ 6.04 }  & & & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}
14h & \multirow{1}{*}{ 6.38 }  & & & & \multirow{1}{*}{ 6.32 }  & & & & \multirow{1}{*}{ 7.09 }  & & & & \multirow{1}{*}{ 6.47 }  & & & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}
15h & \multirow{1}{*}{ 5.93 }  & & & & \multirow{1}{*}{ 5.97 }  & & & & \multirow{1}{*}{ 7.14 }  & & & & \multirow{1}{*}{ 6.10 }  & & & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
16h & \multirow{1}{*}{ 5.52 }  & \multirow{4}{*}{ 20.73 }  & & & \multirow{1}{*}{ 6.40 }  & \multirow{4}{*}{ 23.44 }  & & & \multirow{1}{*}{ 6.68 }  & \multirow{4}{*}{ 24.79 }  & & & \multirow{1}{*}{ 6.22 }  & \multirow{4}{*}{ 23.60 }  & & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}
17h & \multirow{1}{*}{ 5.46 }  & & & & \multirow{1}{*}{ 6.02 }  & & & & \multirow{1}{*}{ 6.89 }  & & & & \multirow{1}{*}{ 6.36 }  & & & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}\cline{3-3}\cline{7-7}\cline{11-11}\cline{15-15}
18h & \multirow{1}{*}{ 5.23 }  & & \multirow{6}{*}{ 27.46 }  & & \multirow{1}{*}{ 5.99 }  & & \multirow{6}{*}{ 29.65 }  & & \multirow{1}{*}{ 5.99 }  & & \multirow{6}{*}{ 28.44 }  & & \multirow{1}{*}{ 6.01 }  & & \multirow{6}{*}{ 28.61 }  & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}
19h & \multirow{1}{*}{ 4.52 }  & & & & \multirow{1}{*}{ 5.03 }  & & & & \multirow{1}{*}{ 5.23 }  & & & & \multirow{1}{*}{ 5.02 }  & & & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
20h & \multirow{1}{*}{ 4.55 }  & \multirow{4}{*}{ 17.71 }  & & & \multirow{1}{*}{ 4.63 }  & \multirow{4}{*}{ 18.63 }  & & & \multirow{1}{*}{ 4.98 }  & \multirow{4}{*}{ 17.22 }  & & & \multirow{1}{*}{ 4.85 }  & \multirow{4}{*}{ 17.59 }  & & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}
21h & \multirow{1}{*}{ 4.42 }  & & & & \multirow{1}{*}{ 4.59 }  & & & & \multirow{1}{*}{ 4.37 }  & & & & \multirow{1}{*}{ 4.38 }  & & & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}
22h & \multirow{1}{*}{ 4.51 }  & & & & \multirow{1}{*}{ 4.88 }  & & & & \multirow{1}{*}{ 4.24 }  & & & & \multirow{1}{*}{ 4.06 }  & & & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}
23h & \multirow{1}{*}{ 4.23 }  & & & & \multirow{1}{*}{ 4.53 }  & & & & \multirow{1}{*}{ 3.64 }  & & & & \multirow{1}{*}{ 4.30 }  & & & \\\cline{1-1}\cline{5-5}\cline{9-9}\cline{13-13}\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}\cline{3-3}\cline{7-7}\cline{11-11}\cline{15-15}\cline{4-4}\cline{8-8}\cline{12-12}\cline{16-16}
\end{tabular}
\end{center}

==> tables/tabHoursCPP.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c | c | c |}\hline
 & 1h & 2h & 3h & 4h & 6h & 12h \\\hline
0h & \multirow{1}{*}{ 3.66 }  & \multirow{2}{*}{ 6.42 }  & \multirow{3}{*}{ 8.20 }  & \multirow{4}{*}{ 9.30 }  & \multirow{6}{*}{ 10.67 }  & \multirow{12}{*}{ 33.76 }  \\\cline{2-2}
1h & \multirow{1}{*}{ 2.76 }  & & & & & \\\cline{2-2}\cline{3-3}
2h & \multirow{1}{*}{ 1.79 }  & \multirow{2}{*}{ 2.88 }  & & & & \\\cline{2-2}\cline{4-4}
3h & \multirow{1}{*}{ 1.10 }  & & \multirow{3}{*}{ 2.47 }  & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
4h & \multirow{1}{*}{ 0.68 }  & \multirow{2}{*}{ 1.37 }  & & \multirow{4}{*}{ 3.44 }  & & \\\cline{2-2}
5h & \multirow{1}{*}{ 0.69 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{6-6}
6h & \multirow{1}{*}{ 0.83 }  & \multirow{2}{*}{ 2.07 }  & \multirow{3}{*}{ 4.35 }  & & \multirow{6}{*}{ 23.09 }  & \\\cline{2-2}
7h & \multirow{1}{*}{ 1.24 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
8h & \multirow{1}{*}{ 2.28 }  & \multirow{2}{*}{ 6.80 }  & & \multirow{4}{*}{ 21.03 }  & & \\\cline{2-2}\cline{4-4}
9h & \multirow{1}{*}{ 4.52 }  & & \multirow{3}{*}{ 18.75 }  & & & \\\cline{2-2}\cline{3-3}
10h & \multirow{1}{*}{ 6.62 }  & \multirow{2}{*}{ 14.23 }  & & & & \\\cline{2-2}
11h & \multirow{1}{*}{ 7.61 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{5-5}\cline{6-6}\cline{7-7}
12h & \multirow{1}{*}{ 6.44 }  & \multirow{2}{*}{ 12.48 }  & \multirow{3}{*}{ 18.95 }  & \multirow{4}{*}{ 25.05 }  & \multirow{6}{*}{ 37.63 }  & \multirow{12}{*}{ 66.24 }  \\\cline{2-2}
13h & \multirow{1}{*}{ 6.04 }  & & & & & \\\cline{2-2}\cline{3-3}
14h & \multirow{1}{*}{ 6.47 }  & \multirow{2}{*}{ 12.57 }  & & & & \\\cline{2-2}\cline{4-4}
15h & \multirow{1}{*}{ 6.10 }  & & \multirow{3}{*}{ 18.68 }  & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
16h & \multirow{1}{*}{ 6.22 }  & \multirow{2}{*}{ 12.58 }  & & \multirow{4}{*}{ 23.60 }  & & \\\cline{2-2}
17h & \multirow{1}{*}{ 6.36 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{6-6}
18h & \multirow{1}{*}{ 6.01 }  & \multirow{2}{*}{ 11.02 }  & \multirow{3}{*}{ 15.88 }  & & \multirow{6}{*}{ 28.61 }  & \\\cline{2-2}
19h & \multirow{1}{*}{ 5.02 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
20h & \multirow{1}{*}{ 4.85 }  & \multirow{2}{*}{ 9.23 }  & & \multirow{4}{*}{ 17.59 }  & & \\\cline{2-2}\cline{4-4}
21h & \multirow{1}{*}{ 4.38 }  & & \multirow{3}{*}{ 12.73 }  & & & \\\cline{2-2}\cline{3-3}
22h & \multirow{1}{*}{ 4.06 }  & \multirow{2}{*}{ 8.36 }  & & & & \\\cline{2-2}
23h & \multirow{1}{*}{ 4.30 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{5-5}\cline{6-6}\cline{7-7}
\hline\end{tabular}
\end{center}

==> tables/tabHoursLAD.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c | c | c |}\hline
 & 1h & 2h & 3h & 4h & 6h & 12h \\\hline
0h & \multirow{1}{*}{ 4.01 }  & \multirow{2}{*}{ 6.53 }  & \multirow{3}{*}{ 8.32 }  & \multirow{4}{*}{ 9.37 }  & \multirow{6}{*}{ 10.78 }  & \multirow{12}{*}{ 33.11 }  \\\cline{2-2}
1h & \multirow{1}{*}{ 2.52 }  & & & & & \\\cline{2-2}\cline{3-3}
2h & \multirow{1}{*}{ 1.79 }  & \multirow{2}{*}{ 2.84 }  & & & & \\\cline{2-2}\cline{4-4}
3h & \multirow{1}{*}{ 1.06 }  & & \multirow{3}{*}{ 2.46 }  & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
4h & \multirow{1}{*}{ 0.75 }  & \multirow{2}{*}{ 1.40 }  & & \multirow{4}{*}{ 3.81 }  & & \\\cline{2-2}
5h & \multirow{1}{*}{ 0.66 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{6-6}
6h & \multirow{1}{*}{ 0.85 }  & \multirow{2}{*}{ 2.41 }  & \multirow{3}{*}{ 5.36 }  & & \multirow{6}{*}{ 22.33 }  & \\\cline{2-2}
7h & \multirow{1}{*}{ 1.56 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
8h & \multirow{1}{*}{ 2.95 }  & \multirow{2}{*}{ 7.61 }  & & \multirow{4}{*}{ 19.93 }  & & \\\cline{2-2}\cline{4-4}
9h & \multirow{1}{*}{ 4.66 }  & & \multirow{3}{*}{ 16.98 }  & & & \\\cline{2-2}\cline{3-3}
10h & \multirow{1}{*}{ 5.92 }  & \multirow{2}{*}{ 12.32 }  & & & & \\\cline{2-2}
11h & \multirow{1}{*}{ 6.40 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{5-5}\cline{6-6}\cline{7-7}
12h & \multirow{1}{*}{ 6.41 }  & \multirow{2}{*}{ 12.53 }  & \multirow{3}{*}{ 18.85 }  & \multirow{4}{*}{ 24.82 }  & \multirow{6}{*}{ 37.24 }  & \multirow{12}{*}{ 66.89 }  \\\cline{2-2}
13h & \multirow{1}{*}{ 6.12 }  & & & & & \\\cline{2-2}\cline{3-3}
14h & \multirow{1}{*}{ 6.32 }  & \multirow{2}{*}{ 12.29 }  & & & & \\\cline{2-2}\cline{4-4}
15h & \multirow{1}{*}{ 5.97 }  & & \multirow{3}{*}{ 18.39 }  & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
16h & \multirow{1}{*}{ 6.40 }  & \multirow{2}{*}{ 12.42 }  & & \multirow{4}{*}{ 23.44 }  & & \\\cline{2-2}
17h & \multirow{1}{*}{ 6.02 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{6-6}
18h & \multirow{1}{*}{ 5.99 }  & \multirow{2}{*}{ 11.02 }  & \multirow{3}{*}{ 15.65 }  & & \multirow{6}{*}{ 29.65 }  & \\\cline{2-2}
19h & \multirow{1}{*}{ 5.03 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
20h & \multirow{1}{*}{ 4.63 }  & \multirow{2}{*}{ 9.22 }  & & \multirow{4}{*}{ 18.63 }  & & \\\cline{2-2}\cline{4-4}
21h & \multirow{1}{*}{ 4.59 }  & & \multirow{3}{*}{ 14.00 }  & & & \\\cline{2-2}\cline{3-3}
22h & \multirow{1}{*}{ 4.88 }  & \multirow{2}{*}{ 9.41 }  & & & & \\\cline{2-2}
23h & \multirow{1}{*}{ 4.53 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{5-5}\cline{6-6}\cline{7-7}
\hline\end{tabular}
\end{center}

==> tables/tabHoursLAU.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c | c | c |}\hline
 & 1h & 2h & 3h & 4h & 6h & 12h \\\hline
0h & \multirow{1}{*}{ 3.58 }  & \multirow{2}{*}{ 5.80 }  & \multirow{3}{*}{ 7.43 }  & \multirow{4}{*}{ 8.49 }  & \multirow{6}{*}{ 10.14 }  & \multirow{12}{*}{ 36.88 }  \\\cline{2-2}
1h & \multirow{1}{*}{ 2.22 }  & & & & & \\\cline{2-2}\cline{3-3}
2h & \multirow{1}{*}{ 1.63 }  & \multirow{2}{*}{ 2.69 }  & & & & \\\cline{2-2}\cline{4-4}
3h & \multirow{1}{*}{ 1.06 }  & & \multirow{3}{*}{ 2.72 }  & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
4h & \multirow{1}{*}{ 0.84 }  & \multirow{2}{*}{ 1.66 }  & & \multirow{4}{*}{ 5.20 }  & & \\\cline{2-2}
5h & \multirow{1}{*}{ 0.82 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{6-6}
6h & \multirow{1}{*}{ 1.17 }  & \multirow{2}{*}{ 3.54 }  & \multirow{3}{*}{ 7.07 }  & & \multirow{6}{*}{ 26.74 }  & \\\cline{2-2}
7h & \multirow{1}{*}{ 2.37 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
8h & \multirow{1}{*}{ 3.53 }  & \multirow{2}{*}{ 9.57 }  & & \multirow{4}{*}{ 23.20 }  & & \\\cline{2-2}\cline{4-4}
9h & \multirow{1}{*}{ 6.04 }  & & \multirow{3}{*}{ 19.67 }  & & & \\\cline{2-2}\cline{3-3}
10h & \multirow{1}{*}{ 6.83 }  & \multirow{2}{*}{ 13.62 }  & & & & \\\cline{2-2}
11h & \multirow{1}{*}{ 6.79 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{5-5}\cline{6-6}\cline{7-7}
12h & \multirow{1}{*}{ 6.11 }  & \multirow{2}{*}{ 12.36 }  & \multirow{3}{*}{ 18.75 }  & \multirow{4}{*}{ 24.68 }  & \multirow{6}{*}{ 35.66 }  & \multirow{12}{*}{ 63.12 }  \\\cline{2-2}
13h & \multirow{1}{*}{ 6.26 }  & & & & & \\\cline{2-2}\cline{3-3}
14h & \multirow{1}{*}{ 6.38 }  & \multirow{2}{*}{ 12.31 }  & & & & \\\cline{2-2}\cline{4-4}
15h & \multirow{1}{*}{ 5.93 }  & & \multirow{3}{*}{ 16.91 }  & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
16h & \multirow{1}{*}{ 5.52 }  & \multirow{2}{*}{ 10.98 }  & & \multirow{4}{*}{ 20.73 }  & & \\\cline{2-2}
17h & \multirow{1}{*}{ 5.46 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{6-6}
18h & \multirow{1}{*}{ 5.23 }  & \multirow{2}{*}{ 9.75 }  & \multirow{3}{*}{ 14.30 }  & & \multirow{6}{*}{ 27.46 }  & \\\cline{2-2}
19h & \multirow{1}{*}{ 4.52 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
20h & \multirow{1}{*}{ 4.55 }  & \multirow{2}{*}{ 8.97 }  & & \multirow{4}{*}{ 17.71 }  & & \\\cline{2-2}\cline{4-4}
21h & \multirow{1}{*}{ 4.42 }  & & \multirow{3}{*}{ 13.16 }  & & & \\\cline{2-2}\cline{3-3}
22h & \multirow{1}{*}{ 4.51 }  & \multirow{2}{*}{ 8.74 }  & & & & \\\cline{2-2}
23h & \multirow{1}{*}{ 4.23 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{5-5}\cline{6-6}\cline{7-7}
\hline\end{tabular}
\end{center}

==> tables/tabHoursMET.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c | c | c |}\hline
 & 1h & 2h & 3h & 4h & 6h & 12h \\\hline
0h & \multirow{1}{*}{ 2.87 }  & \multirow{2}{*}{ 4.64 }  & \multirow{3}{*}{ 5.67 }  & \multirow{4}{*}{ 6.31 }  & \multirow{6}{*}{ 7.15 }  & \multirow{12}{*}{ 29.33 }  \\\cline{2-2}
1h & \multirow{1}{*}{ 1.77 }  & & & & & \\\cline{2-2}\cline{3-3}
2h & \multirow{1}{*}{ 1.04 }  & \multirow{2}{*}{ 1.67 }  & & & & \\\cline{2-2}\cline{4-4}
3h & \multirow{1}{*}{ 0.64 }  & & \multirow{3}{*}{ 1.48 }  & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
4h & \multirow{1}{*}{ 0.47 }  & \multirow{2}{*}{ 0.85 }  & & \multirow{4}{*}{ 2.89 }  & & \\\cline{2-2}
5h & \multirow{1}{*}{ 0.38 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{6-6}
6h & \multirow{1}{*}{ 0.72 }  & \multirow{2}{*}{ 2.04 }  & \multirow{3}{*}{ 4.71 }  & & \multirow{6}{*}{ 22.18 }  & \\\cline{2-2}
7h & \multirow{1}{*}{ 1.33 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
8h & \multirow{1}{*}{ 2.67 }  & \multirow{2}{*}{ 7.07 }  & & \multirow{4}{*}{ 20.14 }  & & \\\cline{2-2}\cline{4-4}
9h & \multirow{1}{*}{ 4.40 }  & & \multirow{3}{*}{ 17.47 }  & & & \\\cline{2-2}\cline{3-3}
10h & \multirow{1}{*}{ 6.29 }  & \multirow{2}{*}{ 13.07 }  & & & & \\\cline{2-2}
11h & \multirow{1}{*}{ 6.78 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{5-5}\cline{6-6}\cline{7-7}
12h & \multirow{1}{*}{ 7.33 }  & \multirow{2}{*}{ 14.41 }  & \multirow{3}{*}{ 21.50 }  & \multirow{4}{*}{ 28.65 }  & \multirow{6}{*}{ 42.22 }  & \multirow{12}{*}{ 70.67 }  \\\cline{2-2}
13h & \multirow{1}{*}{ 7.08 }  & & & & & \\\cline{2-2}\cline{3-3}
14h & \multirow{1}{*}{ 7.09 }  & \multirow{2}{*}{ 14.24 }  & & & & \\\cline{2-2}\cline{4-4}
15h & \multirow{1}{*}{ 7.14 }  & & \multirow{3}{*}{ 20.72 }  & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
16h & \multirow{1}{*}{ 6.68 }  & \multirow{2}{*}{ 13.58 }  & & \multirow{4}{*}{ 24.79 }  & & \\\cline{2-2}
17h & \multirow{1}{*}{ 6.89 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{6-6}
18h & \multirow{1}{*}{ 5.99 }  & \multirow{2}{*}{ 11.22 }  & \multirow{3}{*}{ 16.19 }  & & \multirow{6}{*}{ 28.44 }  & \\\cline{2-2}
19h & \multirow{1}{*}{ 5.23 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
20h & \multirow{1}{*}{ 4.98 }  & \multirow{2}{*}{ 9.34 }  & & \multirow{4}{*}{ 17.22 }  & & \\\cline{2-2}\cline{4-4}
21h & \multirow{1}{*}{ 4.37 }  & & \multirow{3}{*}{ 12.25 }  & & & \\\cline{2-2}\cline{3-3}
22h & \multirow{1}{*}{ 4.24 }  & \multirow{2}{*}{ 7.88 }  & & & & \\\cline{2-2}
23h & \multirow{1}{*}{ 3.64 }  & & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{5-5}\cline{6-6}\cline{7-7}
\hline\end{tabular}
\end{center}

==> tables/tabMonthdaysALL.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |}\hline
 & \multicolumn{4}{c|}{LAU} & \multicolumn{4}{c|}{LAD} & \multicolumn{4}{c|}{MET} & \multicolumn{4}{c|}{CPP} \\\hline
 & 1 day & 5 days & 10 days & 15 days & 1 day & 5 days & 10 days & 15 days & 1 day & 5 days & 10 days & 15 days & 1 day & 5 days & 10 days & 15 days \\\hline
1 & \multirow{1}{*}{ 3.36 }  & \multirow{5}{*}{ 16.21 }  & \multirow{10}{*}{ 33.71 }  & \multirow{15}{*}{ 50.82 }  & \multirow{1}{*}{ 3.29 }  & \multirow{5}{*}{ 15.77 }  & \multirow{10}{*}{ 33.63 }  & \multirow{15}{*}{ 50.50 }  & \multirow{1}{*}{ 3.05 }  & \multirow{5}{*}{ 18.25 }  & \multirow{10}{*}{ 35.24 }  & \multirow{15}{*}{ 50.96 }  & \multirow{1}{*}{ 3.22 }  & \multirow{5}{*}{ 15.98 }  & \multirow{10}{*}{ 31.82 }  & \multirow{15}{*}{ 49.62 }  \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
2 & \multirow{1}{*}{ 3.43 }  & & & & \multirow{1}{*}{ 3.38 }  & & & & \multirow{1}{*}{ 3.38 }  & & & & \multirow{1}{*}{ 3.08 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
3 & \multirow{1}{*}{ 3.31 }  & & & & \multirow{1}{*}{ 2.85 }  & & & & \multirow{1}{*}{ 3.62 }  & & & & \multirow{1}{*}{ 3.19 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
4 & \multirow{1}{*}{ 3.37 }  & & & & \multirow{1}{*}{ 2.94 }  & & & & \multirow{1}{*}{ 4.25 }  & & & & \multirow{1}{*}{ 3.65 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
5 & \multirow{1}{*}{ 2.75 }  & & & & \multirow{1}{*}{ 3.31 }  & & & & \multirow{1}{*}{ 3.94 }  & & & & \multirow{1}{*}{ 2.84 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}\cline{3-3}\cline{7-7}\cline{11-11}\cline{15-15}
6 & \multirow{1}{*}{ 3.03 }  & \multirow{5}{*}{ 17.50 }  & & & \multirow{1}{*}{ 3.60 }  & \multirow{5}{*}{ 17.85 }  & & & \multirow{1}{*}{ 3.73 }  & \multirow{5}{*}{ 16.98 }  & & & \multirow{1}{*}{ 3.65 }  & \multirow{5}{*}{ 15.84 }  & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
7 & \multirow{1}{*}{ 3.93 }  & & & & \multirow{1}{*}{ 2.68 }  & & & & \multirow{1}{*}{ 3.17 }  & & & & \multirow{1}{*}{ 3.53 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
8 & \multirow{1}{*}{ 3.62 }  & & & & \multirow{1}{*}{ 3.78 }  & & & & \multirow{1}{*}{ 3.26 }  & & & & \multirow{1}{*}{ 3.10 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
9 & \multirow{1}{*}{ 3.84 }  & & & & \multirow{1}{*}{ 3.88 }  & & & & \multirow{1}{*}{ 3.56 }  & & & & \multirow{1}{*}{ 2.49 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
10 & \multirow{1}{*}{ 3.09 }  & & & & \multirow{1}{*}{ 3.91 }  & & & & \multirow{1}{*}{ 3.26 }  & & & & \multirow{1}{*}{ 3.07 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}\cline{3-3}\cline{7-7}\cline{11-11}\cline{15-15}\cline{4-4}\cline{8-8}\cline{12-12}\cline{16-16}
11 & \multirow{1}{*}{ 3.20 }  & \multirow{5}{*}{ 17.11 }  & \multirow{10}{*}{ 34.02 }  & & \multirow{1}{*}{ 3.22 }  & \multirow{5}{*}{ 16.87 }  & \multirow{10}{*}{ 33.41 }  & & \multirow{1}{*}{ 3.81 }  & \multirow{5}{*}{ 15.73 }  & \multirow{10}{*}{ 31.98 }  & & \multirow{1}{*}{ 3.47 }  & \multirow{5}{*}{ 17.80 }  & \multirow{10}{*}{ 34.22 }  & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
12 & \multirow{1}{*}{ 3.40 }  & & & & \multirow{1}{*}{ 2.79 }  & & & & \multirow{1}{*}{ 2.91 }  & & & & \multirow{1}{*}{ 3.26 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
13 & \multirow{1}{*}{ 3.67 }  & & & & \multirow{1}{*}{ 3.50 }  & & & & \multirow{1}{*}{ 3.30 }  & & & & \multirow{1}{*}{ 3.55 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
14 & \multirow{1}{*}{ 3.71 }  & & & & \multirow{1}{*}{ 3.95 }  & & & & \multirow{1}{*}{ 2.75 }  & & & & \multirow{1}{*}{ 3.84 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
15 & \multirow{1}{*}{ 3.14 }  & & & & \multirow{1}{*}{ 3.40 }  & & & & \multirow{1}{*}{ 2.95 }  & & & & \multirow{1}{*}{ 3.68 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}\cline{3-3}\cline{7-7}\cline{11-11}\cline{15-15}\cline{5-5}\cline{9-9}\cline{13-13}\cline{17-17}
16 & \multirow{1}{*}{ 3.08 }  & \multirow{5}{*}{ 16.91 }  & & \multirow{15}{*}{ 49.18 }  & \multirow{1}{*}{ 3.32 }  & \multirow{5}{*}{ 16.54 }  & & \multirow{15}{*}{ 49.50 }  & \multirow{1}{*}{ 3.36 }  & \multirow{5}{*}{ 16.25 }  & & \multirow{15}{*}{ 49.04 }  & \multirow{1}{*}{ 3.74 }  & \multirow{5}{*}{ 16.42 }  & & \multirow{15}{*}{ 50.38 }  \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
17 & \multirow{1}{*}{ 3.13 }  & & & & \multirow{1}{*}{ 2.95 }  & & & & \multirow{1}{*}{ 3.16 }  & & & & \multirow{1}{*}{ 3.40 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
18 & \multirow{1}{*}{ 3.43 }  & & & & \multirow{1}{*}{ 3.50 }  & & & & \multirow{1}{*}{ 3.44 }  & & & & \multirow{1}{*}{ 3.41 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
19 & \multirow{1}{*}{ 3.61 }  & & & & \multirow{1}{*}{ 3.69 }  & & & & \multirow{1}{*}{ 3.36 }  & & & & \multirow{1}{*}{ 2.95 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
20 & \multirow{1}{*}{ 3.67 }  & & & & \multirow{1}{*}{ 3.07 }  & & & & \multirow{1}{*}{ 2.93 }  & & & & \multirow{1}{*}{ 2.93 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}\cline{3-3}\cline{7-7}\cline{11-11}\cline{15-15}\cline{4-4}\cline{8-8}\cline{12-12}\cline{16-16}
21 & \multirow{1}{*}{ 3.60 }  & \multirow{5}{*}{ 15.43 }  & \multirow{10}{*}{ 32.27 }  & & \multirow{1}{*}{ 2.76 }  & \multirow{5}{*}{ 15.71 }  & \multirow{10}{*}{ 32.96 }  & & \multirow{1}{*}{ 3.20 }  & \multirow{5}{*}{ 15.79 }  & \multirow{10}{*}{ 32.78 }  & & \multirow{1}{*}{ 3.15 }  & \multirow{5}{*}{ 17.13 }  & \multirow{10}{*}{ 33.96 }  & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
22 & \multirow{1}{*}{ 3.42 }  & & & & \multirow{1}{*}{ 3.35 }  & & & & \multirow{1}{*}{ 3.11 }  & & & & \multirow{1}{*}{ 3.64 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
23 & \multirow{1}{*}{ 2.80 }  & & & & \multirow{1}{*}{ 3.32 }  & & & & \multirow{1}{*}{ 3.60 }  & & & & \multirow{1}{*}{ 3.51 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
24 & \multirow{1}{*}{ 2.64 }  & & & & \multirow{1}{*}{ 3.15 }  & & & & \multirow{1}{*}{ 2.74 }  & & & & \multirow{1}{*}{ 3.32 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
25 & \multirow{1}{*}{ 2.97 }  & & & & \multirow{1}{*}{ 3.13 }  & & & & \multirow{1}{*}{ 3.13 }  & & & & \multirow{1}{*}{ 3.51 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}\cline{3-3}\cline{7-7}\cline{11-11}\cline{15-15}
26 & \multirow{1}{*}{ 3.06 }  & \multirow{5}{*}{ 16.85 }  & & & \multirow{1}{*}{ 3.68 }  & \multirow{5}{*}{ 17.25 }  & & & \multirow{1}{*}{ 3.13 }  & \multirow{5}{*}{ 16.99 }  & & & \multirow{1}{*}{ 3.54 }  & \multirow{5}{*}{ 16.84 }  & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
27 & \multirow{1}{*}{ 2.69 }  & & & & \multirow{1}{*}{ 4.02 }  & & & & \multirow{1}{*}{ 3.07 }  & & & & \multirow{1}{*}{ 3.21 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
28 & \multirow{1}{*}{ 3.79 }  & & & & \multirow{1}{*}{ 3.49 }  & & & & \multirow{1}{*}{ 3.61 }  & & & & \multirow{1}{*}{ 3.40 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
29 & \multirow{1}{*}{ 3.75 }  & & & & \multirow{1}{*}{ 3.34 }  & & & & \multirow{1}{*}{ 3.60 }  & & & & \multirow{1}{*}{ 3.83 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}
30 & \multirow{1}{*}{ 3.57 }  & & & & \multirow{1}{*}{ 2.72 }  & & & & \multirow{1}{*}{ 3.57 }  & & & & \multirow{1}{*}{ 2.86 }  & & & \\\cline{2-2}\cline{6-6}\cline{10-10}\cline{14-14}\cline{3-3}\cline{7-7}\cline{11-11}\cline{15-15}\cline{4-4}\cline{8-8}\cline{12-12}\cline{16-16}\cline{5-5}\cline{9-9}\cline{13-13}\cline{17-17}
\hline\end{tabular}
\end{center}

==> tables/tabMonthdaysCPP.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c |}\hline
 & 1 day & 5 & 10 & 15 days \\\hline
1 & \multirow{1}{*}{ 3.22 }  & \multirow{5}{*}{ 15.98 }  & \multirow{10}{*}{ 31.82 }  & \multirow{15}{*}{ 49.62 }  \\\cline{2-2}
2 & \multirow{1}{*}{ 3.08 }  & & & \\\cline{2-2}
3 & \multirow{1}{*}{ 3.19 }  & & & \\\cline{2-2}
4 & \multirow{1}{*}{ 3.65 }  & & & \\\cline{2-2}
5 & \multirow{1}{*}{ 2.84 }  & & & \\\cline{2-2}\cline{3-3}
6 & \multirow{1}{*}{ 3.65 }  & \multirow{5}{*}{ 15.84 }  & & \\\cline{2-2}
7 & \multirow{1}{*}{ 3.53 }  & & & \\\cline{2-2}
8 & \multirow{1}{*}{ 3.10 }  & & & \\\cline{2-2}
9 & \multirow{1}{*}{ 2.49 }  & & & \\\cline{2-2}
10 & \multirow{1}{*}{ 3.07 }  & & & \\\cline{2-2}\cline{3-3}\cline{4-4}
11 & \multirow{1}{*}{ 3.47 }  & \multirow{5}{*}{ 17.80 }  & \multirow{10}{*}{ 34.22 }  & \\\cline{2-2}
12 & \multirow{1}{*}{ 3.26 }  & & & \\\cline{2-2}
13 & \multirow{1}{*}{ 3.55 }  & & & \\\cline{2-2}
14 & \multirow{1}{*}{ 3.84 }  & & & \\\cline{2-2}
15 & \multirow{1}{*}{ 3.68 }  & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
16 & \multirow{1}{*}{ 3.74 }  & \multirow{5}{*}{ 16.42 }  & & \multirow{15}{*}{ 50.38 }  \\\cline{2-2}
17 & \multirow{1}{*}{ 3.40 }  & & & \\\cline{2-2}
18 & \multirow{1}{*}{ 3.41 }  & & & \\\cline{2-2}
19 & \multirow{1}{*}{ 2.95 }  & & & \\\cline{2-2}
20 & \multirow{1}{*}{ 2.93 }  & & & \\\cline{2-2}\cline{3-3}\cline{4-4}
21 & \multirow{1}{*}{ 3.15 }  & \multirow{5}{*}{ 17.13 }  & \multirow{10}{*}{ 33.96 }  & \\\cline{2-2}
22 & \multirow{1}{*}{ 3.64 }  & & & \\\cline{2-2}
23 & \multirow{1}{*}{ 3.51 }  & & & \\\cline{2-2}
24 & \multirow{1}{*}{ 3.32 }  & & & \\\cline{2-2}
25 & \multirow{1}{*}{ 3.51 }  & & & \\\cline{2-2}\cline{3-3}
26 & \multirow{1}{*}{ 3.54 }  & \multirow{5}{*}{ 16.84 }  & & \\\cline{2-2}
27 & \multirow{1}{*}{ 3.21 }  & & & \\\cline{2-2}
28 & \multirow{1}{*}{ 3.40 }  & & & \\\cline{2-2}
29 & \multirow{1}{*}{ 3.83 }  & & & \\\cline{2-2}
30 & \multirow{1}{*}{ 2.86 }  & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{5-5}
\hline\end{tabular}
\end{center}

==> tables/tabMonthdaysLAD.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c |}\hline
 & 1 day & 5 & 10 & 15 days \\\hline
1 & \multirow{1}{*}{ 3.29 }  & \multirow{5}{*}{ 15.77 }  & \multirow{10}{*}{ 33.63 }  & \multirow{15}{*}{ 50.50 }  \\\cline{2-2}
2 & \multirow{1}{*}{ 3.38 }  & & & \\\cline{2-2}
3 & \multirow{1}{*}{ 2.85 }  & & & \\\cline{2-2}
4 & \multirow{1}{*}{ 2.94 }  & & & \\\cline{2-2}
5 & \multirow{1}{*}{ 3.31 }  & & & \\\cline{2-2}\cline{3-3}
6 & \multirow{1}{*}{ 3.60 }  & \multirow{5}{*}{ 17.85 }  & & \\\cline{2-2}
7 & \multirow{1}{*}{ 2.68 }  & & & \\\cline{2-2}
8 & \multirow{1}{*}{ 3.78 }  & & & \\\cline{2-2}
9 & \multirow{1}{*}{ 3.88 }  & & & \\\cline{2-2}
10 & \multirow{1}{*}{ 3.91 }  & & & \\\cline{2-2}\cline{3-3}\cline{4-4}
11 & \multirow{1}{*}{ 3.22 }  & \multirow{5}{*}{ 16.87 }  & \multirow{10}{*}{ 33.41 }  & \\\cline{2-2}
12 & \multirow{1}{*}{ 2.79 }  & & & \\\cline{2-2}
13 & \multirow{1}{*}{ 3.50 }  & & & \\\cline{2-2}
14 & \multirow{1}{*}{ 3.95 }  & & & \\\cline{2-2}
15 & \multirow{1}{*}{ 3.40 }  & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
16 & \multirow{1}{*}{ 3.32 }  & \multirow{5}{*}{ 16.54 }  & & \multirow{15}{*}{ 49.50 }  \\\cline{2-2}
17 & \multirow{1}{*}{ 2.95 }  & & & \\\cline{2-2}
18 & \multirow{1}{*}{ 3.50 }  & & & \\\cline{2-2}
19 & \multirow{1}{*}{ 3.69 }  & & & \\\cline{2-2}
20 & \multirow{1}{*}{ 3.07 }  & & & \\\cline{2-2}\cline{3-3}\cline{4-4}
21 & \multirow{1}{*}{ 2.76 }  & \multirow{5}{*}{ 15.71 }  & \multirow{10}{*}{ 32.96 }  & \\\cline{2-2}
22 & \multirow{1}{*}{ 3.35 }  & & & \\\cline{2-2}
23 & \multirow{1}{*}{ 3.32 }  & & & \\\cline{2-2}
24 & \multirow{1}{*}{ 3.15 }  & & & \\\cline{2-2}
25 & \multirow{1}{*}{ 3.13 }  & & & \\\cline{2-2}\cline{3-3}
26 & \multirow{1}{*}{ 3.68 }  & \multirow{5}{*}{ 17.25 }  & & \\\cline{2-2}
27 & \multirow{1}{*}{ 4.02 }  & & & \\\cline{2-2}
28 & \multirow{1}{*}{ 3.49 }  & & & \\\cline{2-2}
29 & \multirow{1}{*}{ 3.34 }  & & & \\\cline{2-2}
30 & \multirow{1}{*}{ 2.72 }  & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{5-5}
\hline\end{tabular}
\end{center}

==> tables/tabMonthdaysLAU.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c |}\hline
 & 1 day & 5 & 10 & 15 days \\\hline
1 & \multirow{1}{*}{ 3.36 }  & \multirow{5}{*}{ 16.21 }  & \multirow{10}{*}{ 33.71 }  & \multirow{15}{*}{ 50.82 }  \\\cline{2-2}
2 & \multirow{1}{*}{ 3.43 }  & & & \\\cline{2-2}
3 & \multirow{1}{*}{ 3.31 }  & & & \\\cline{2-2}
4 & \multirow{1}{*}{ 3.37 }  & & & \\\cline{2-2}
5 & \multirow{1}{*}{ 2.75 }  & & & \\\cline{2-2}\cline{3-3}
6 & \multirow{1}{*}{ 3.03 }  & \multirow{5}{*}{ 17.50 }  & & \\\cline{2-2}
7 & \multirow{1}{*}{ 3.93 }  & & & \\\cline{2-2}
8 & \multirow{1}{*}{ 3.62 }  & & & \\\cline{2-2}
9 & \multirow{1}{*}{ 3.84 }  & & & \\\cline{2-2}
10 & \multirow{1}{*}{ 3.09 }  & & & \\\cline{2-2}\cline{3-3}\cline{4-4}
11 & \multirow{1}{*}{ 3.20 }  & \multirow{5}{*}{ 17.11 }  & \multirow{10}{*}{ 34.02 }  & \\\cline{2-2}
12 & \multirow{1}{*}{ 3.40 }  & & & \\\cline{2-2}
13 & \multirow{1}{*}{ 3.67 }  & & & \\\cline{2-2}
14 & \multirow{1}{*}{ 3.71 }  & & & \\\cline{2-2}
15 & \multirow{1}{*}{ 3.14 }  & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
16 & \multirow{1}{*}{ 3.08 }  & \multirow{5}{*}{ 16.91 }  & & \multirow{15}{*}{ 49.18 }  \\\cline{2-2}
17 & \multirow{1}{*}{ 3.13 }  & & & \\\cline{2-2}
18 & \multirow{1}{*}{ 3.43 }  & & & \\\cline{2-2}
19 & \multirow{1}{*}{ 3.61 }  & & & \\\cline{2-2}
20 & \multirow{1}{*}{ 3.67 }  & & & \\\cline{2-2}\cline{3-3}\cline{4-4}
21 & \multirow{1}{*}{ 3.60 }  & \multirow{5}{*}{ 15.43 }  & \multirow{10}{*}{ 32.27 }  & \\\cline{2-2}
22 & \multirow{1}{*}{ 3.42 }  & & & \\\cline{2-2}
23 & \multirow{1}{*}{ 2.80 }  & & & \\\cline{2-2}
24 & \multirow{1}{*}{ 2.64 }  & & & \\\cline{2-2}
25 & \multirow{1}{*}{ 2.97 }  & & & \\\cline{2-2}\cline{3-3}
26 & \multirow{1}{*}{ 3.06 }  & \multirow{5}{*}{ 16.85 }  & & \\\cline{2-2}
27 & \multirow{1}{*}{ 2.69 }  & & & \\\cline{2-2}
28 & \multirow{1}{*}{ 3.79 }  & & & \\\cline{2-2}
29 & \multirow{1}{*}{ 3.75 }  & & & \\\cline{2-2}
30 & \multirow{1}{*}{ 3.57 }  & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{5-5}
\hline\end{tabular}
\end{center}

==> tables/tabMonthsALL.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |}\hline
 & \multicolumn{5}{c|}{LAU} & \multicolumn{5}{c|}{LAD} & \multicolumn{5}{c|}{MET} & \multicolumn{5}{c|}{CPP} \\\hline
 & m. & b. & t. & q. & s. & m. & b. & t. & q. & s. & m. & b. & t. & q. & s. & m. & b. & t. & q. & s. \\\hline
Jan & \multirow{1}{*}{ 10.22 }  & \multirow{2}{*}{ 19.56 }  & \multirow{3}{*}{ 28.24 }  & \multirow{4}{*}{ 35.09 }  & \multirow{6}{*}{ 49.16 }  & \multirow{1}{*}{ 11.24 }  & \multirow{2}{*}{ 18.51 }  & \multirow{3}{*}{ 26.46 }  & \multirow{4}{*}{ 36.07 }  & \multirow{6}{*}{ 57.96 }  & \multirow{1}{*}{ 4.87 }  & \multirow{2}{*}{ 11.00 }  & \multirow{3}{*}{ 16.89 }  & \multirow{4}{*}{ 23.30 }  & \multirow{6}{*}{ 47.70 }  & \multirow{1}{*}{ 8.70 }  & \multirow{2}{*}{ 17.00 }  & \multirow{3}{*}{ 27.23 }  & \multirow{4}{*}{ 36.49 }  & \multirow{6}{*}{ 54.27 }  \\\cline{2-2}\cline{7-7}\cline{12-12}\cline{17-17}
Fev & \multirow{1}{*}{ 9.34 }  & & & & & \multirow{1}{*}{ 7.26 }  & & & & & \multirow{1}{*}{ 6.13 }  & & & & & \multirow{1}{*}{ 8.29 }  & & & & \\\cline{2-2}\cline{7-7}\cline{12-12}\cline{17-17}\cline{3-3}\cline{8-8}\cline{13-13}\cline{18-18}
Mar & \multirow{1}{*}{ 8.67 }  & \multirow{2}{*}{ 15.53 }  & & & & \multirow{1}{*}{ 7.95 }  & \multirow{2}{*}{ 17.56 }  & & & & \multirow{1}{*}{ 5.89 }  & \multirow{2}{*}{ 12.30 }  & & & & \multirow{1}{*}{ 10.23 }  & \multirow{2}{*}{ 19.49 }  & & & \\\cline{2-2}\cline{7-7}\cline{12-12}\cline{17-17}\cline{4-4}\cline{9-9}\cline{14-14}\cline{19-19}
Apr & \multirow{1}{*}{ 6.86 }  & & \multirow{3}{*}{ 20.93 }  & & & \multirow{1}{*}{ 9.61 }  & & \multirow{3}{*}{ 31.50 }  & & & \multirow{1}{*}{ 6.41 }  & & \multirow{3}{*}{ 30.81 }  & & & \multirow{1}{*}{ 9.26 }  & & \multirow{3}{*}{ 27.03 }  & & \\\cline{2-2}\cline{7-7}\cline{12-12}\cline{17-17}\cline{3-3}\cline{8-8}\cline{13-13}\cline{18-18}\cline{5-5}\cline{10-10}\cline{15-15}\cline{20-20}
Mai & \multirow{1}{*}{ 7.28 }  & \multirow{2}{*}{ 14.07 }  & & \multirow{4}{*}{ 30.36 }  & & \multirow{1}{*}{ 8.94 }  & \multirow{2}{*}{ 21.89 }  & & \multirow{4}{*}{ 37.56 }  & & \multirow{1}{*}{ 10.45 }  & \multirow{2}{*}{ 24.40 }  & & \multirow{4}{*}{ 47.87 }  & & \multirow{1}{*}{ 9.41 }  & \multirow{2}{*}{ 17.78 }  & & \multirow{4}{*}{ 33.46 }  & \\\cline{2-2}\cline{7-7}\cline{12-12}\cline{17-17}
Jun & \multirow{1}{*}{ 6.80 }  & & & & & \multirow{1}{*}{ 12.95 }  & & & & & \multirow{1}{*}{ 13.95 }  & & & & & \multirow{1}{*}{ 8.37 }  & & & & \\\cline{2-2}\cline{7-7}\cline{12-12}\cline{17-17}\cline{3-3}\cline{8-8}\cline{13-13}\cline{18-18}\cline{4-4}\cline{9-9}\cline{14-14}\cline{19-19}\cline{6-6}\cline{11-11}\cline{16-16}\cline{21-21}
Jul & \multirow{1}{*}{ 8.97 }  & \multirow{2}{*}{ 16.29 }  & \multirow{3}{*}{ 24.47 }  & & \multirow{6}{*}{ 50.84 }  & \multirow{1}{*}{ 9.03 }  & \multirow{2}{*}{ 15.67 }  & \multirow{3}{*}{ 22.30 }  & & \multirow{6}{*}{ 42.04 }  & \multirow{1}{*}{ 13.24 }  & \multirow{2}{*}{ 23.47 }  & \multirow{3}{*}{ 31.21 }  & & \multirow{6}{*}{ 52.30 }  & \multirow{1}{*}{ 8.70 }  & \multirow{2}{*}{ 15.68 }  & \multirow{3}{*}{ 22.94 }  & & \multirow{6}{*}{ 45.73 }  \\\cline{2-2}\cline{7-7}\cline{12-12}\cline{17-17}
Ago & \multirow{1}{*}{ 7.32 }  & & & & & \multirow{1}{*}{ 6.64 }  & & & & & \multirow{1}{*}{ 10.22 }  & & & & & \multirow{1}{*}{ 6.98 }  & & & & \\\cline{2-2}\cline{7-7}\cline{12-12}\cline{17-17}\cline{3-3}\cline{8-8}\cline{13-13}\cline{18-18}\cline{5-5}\cline{10-10}\cline{15-15}\cline{20-20}
Set & \multirow{1}{*}{ 8.18 }  & \multirow{2}{*}{ 16.25 }  & & \multirow{4}{*}{ 34.55 }  & & \multirow{1}{*}{ 6.63 }  & \multirow{2}{*}{ 12.38 }  & & \multirow{4}{*}{ 26.37 }  & & \multirow{1}{*}{ 7.75 }  & \multirow{2}{*}{ 16.79 }  & & \multirow{4}{*}{ 28.83 }  & & \multirow{1}{*}{ 7.26 }  & \multirow{2}{*}{ 15.36 }  & & \multirow{4}{*}{ 30.06 }  & \\\cline{2-2}\cline{7-7}\cline{12-12}\cline{17-17}\cline{4-4}\cline{9-9}\cline{14-14}\cline{19-19}
Out & \multirow{1}{*}{ 8.06 }  & & \multirow{3}{*}{ 26.36 }  & & & \multirow{1}{*}{ 5.75 }  & & \multirow{3}{*}{ 19.74 }  & & & \multirow{1}{*}{ 9.04 }  & & \multirow{3}{*}{ 21.09 }  & & & \multirow{1}{*}{ 8.10 }  & & \multirow{3}{*}{ 22.80 }  & & \\\cline{2-2}\cline{7-7}\cline{12-12}\cline{17-17}\cline{3-3}\cline{8-8}\cline{13-13}\cline{18-18}
Nov & \multirow{1}{*}{ 7.64 }  & \multirow{2}{*}{ 18.30 }  & & & & \multirow{1}{*}{ 7.61 }  & \multirow{2}{*}{ 13.99 }  & & & & \multirow{1}{*}{ 7.45 }  & \multirow{2}{*}{ 12.05 }  & & & & \multirow{1}{*}{ 7.89 }  & \multirow{2}{*}{ 14.69 }  & & & \\\cline{2-2}\cline{7-7}\cline{12-12}\cline{17-17}
Dez & \multirow{1}{*}{ 10.66 }  & & & & & \multirow{1}{*}{ 6.38 }  & & & & & \multirow{1}{*}{ 4.59 }  & & & & & \multirow{1}{*}{ 6.81 }  & & & & \\\cline{2-2}\cline{7-7}\cline{12-12}\cline{17-17}\cline{3-3}\cline{8-8}\cline{13-13}\cline{18-18}\cline{4-4}\cline{9-9}\cline{14-14}\cline{19-19}\cline{5-5}\cline{10-10}\cline{15-15}\cline{20-20}\cline{6-6}\cline{11-11}\cline{16-16}\cline{21-21}
\hline\end{tabular}
\end{center}

==> tables/tabMonthsCPP.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c | c |}\hline
 & m. & b. & t. & q. & s. \\\hline
Jan & \multirow{1}{*}{ 8.70 }  & \multirow{2}{*}{ 17.00 }  & \multirow{3}{*}{ 27.23 }  & \multirow{4}{*}{ 36.49 }  & \multirow{6}{*}{ 54.27 }  \\\cline{2-2}
Fev & \multirow{1}{*}{ 8.29 }  & & & & \\\cline{2-2}\cline{3-3}
Mar & \multirow{1}{*}{ 10.23 }  & \multirow{2}{*}{ 19.49 }  & & & \\\cline{2-2}\cline{4-4}
Apr & \multirow{1}{*}{ 9.26 }  & & \multirow{3}{*}{ 27.03 }  & & \\\cline{2-2}\cline{3-3}\cline{5-5}
Mai & \multirow{1}{*}{ 9.41 }  & \multirow{2}{*}{ 17.78 }  & & \multirow{4}{*}{ 33.46 }  & \\\cline{2-2}
Jun & \multirow{1}{*}{ 8.37 }  & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{6-6}
Jul & \multirow{1}{*}{ 8.70 }  & \multirow{2}{*}{ 15.68 }  & \multirow{3}{*}{ 22.94 }  & & \multirow{6}{*}{ 45.73 }  \\\cline{2-2}
Ago & \multirow{1}{*}{ 6.98 }  & & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
Set & \multirow{1}{*}{ 7.26 }  & \multirow{2}{*}{ 15.36 }  & & \multirow{4}{*}{ 30.06 }  & \\\cline{2-2}\cline{4-4}
Out & \multirow{1}{*}{ 8.10 }  & & \multirow{3}{*}{ 22.80 }  & & \\\cline{2-2}\cline{3-3}
Nov & \multirow{1}{*}{ 7.89 }  & \multirow{2}{*}{ 14.69 }  & & & \\\cline{2-2}
Dez & \multirow{1}{*}{ 6.81 }  & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{5-5}\cline{6-6}
\hline\end{tabular}
\end{center}

==> tables/tabMonthsLAD.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c | c |}\hline
 & m. & b. & t. & q. & s. \\\hline
Jan & \multirow{1}{*}{ 11.24 }  & \multirow{2}{*}{ 18.51 }  & \multirow{3}{*}{ 26.46 }  & \multirow{4}{*}{ 36.07 }  & \multirow{6}{*}{ 57.96 }  \\\cline{2-2}
Fev & \multirow{1}{*}{ 7.26 }  & & & & \\\cline{2-2}\cline{3-3}
Mar & \multirow{1}{*}{ 7.95 }  & \multirow{2}{*}{ 17.56 }  & & & \\\cline{2-2}\cline{4-4}
Apr & \multirow{1}{*}{ 9.61 }  & & \multirow{3}{*}{ 31.50 }  & & \\\cline{2-2}\cline{3-3}\cline{5-5}
Mai & \multirow{1}{*}{ 8.94 }  & \multirow{2}{*}{ 21.89 }  & & \multirow{4}{*}{ 37.56 }  & \\\cline{2-2}
Jun & \multirow{1}{*}{ 12.95 }  & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{6-6}
Jul & \multirow{1}{*}{ 9.03 }  & \multirow{2}{*}{ 15.67 }  & \multirow{3}{*}{ 22.30 }  & & \multirow{6}{*}{ 42.04 }  \\\cline{2-2}
Ago & \multirow{1}{*}{ 6.64 }  & & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
Set & \multirow{1}{*}{ 6.63 }  & \multirow{2}{*}{ 12.38 }  & & \multirow{4}{*}{ 26.37 }  & \\\cline{2-2}\cline{4-4}
Out & \multirow{1}{*}{ 5.75 }  & & \multirow{3}{*}{ 19.74 }  & & \\\cline{2-2}\cline{3-3}
Nov & \multirow{1}{*}{ 7.61 }  & \multirow{2}{*}{ 13.99 }  & & & \\\cline{2-2}
Dez & \multirow{1}{*}{ 6.38 }  & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{5-5}\cline{6-6}
\hline\end{tabular}
\end{center}

==> tables/tabMonthsMET.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c | c |}\hline
 & m. & b. & t. & q. & s. \\\hline
Jan & \multirow{1}{*}{ 4.87 }  & \multirow{2}{*}{ 11.00 }  & \multirow{3}{*}{ 16.89 }  & \multirow{4}{*}{ 23.30 }  & \multirow{6}{*}{ 47.70 }  \\\cline{2-2}
Fev & \multirow{1}{*}{ 6.13 }  & & & & \\\cline{2-2}\cline{3-3}
Mar & \multirow{1}{*}{ 5.89 }  & \multirow{2}{*}{ 12.30 }  & & & \\\cline{2-2}\cline{4-4}
Apr & \multirow{1}{*}{ 6.41 }  & & \multirow{3}{*}{ 30.81 }  & & \\\cline{2-2}\cline{3-3}\cline{5-5}
Mai & \multirow{1}{*}{ 10.45 }  & \multirow{2}{*}{ 24.40 }  & & \multirow{4}{*}{ 47.87 }  & \\\cline{2-2}
Jun & \multirow{1}{*}{ 13.95 }  & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{6-6}
Jul & \multirow{1}{*}{ 13.24 }  & \multirow{2}{*}{ 23.47 }  & \multirow{3}{*}{ 31.21 }  & & \multirow{6}{*}{ 52.30 }  \\\cline{2-2}
Ago & \multirow{1}{*}{ 10.22 }  & & & & \\\cline{2-2}\cline{3-3}\cline{5-5}
Set & \multirow{1}{*}{ 7.75 }  & \multirow{2}{*}{ 16.79 }  & & \multirow{4}{*}{ 28.83 }  & \\\cline{2-2}\cline{4-4}
Out & \multirow{1}{*}{ 9.04 }  & & \multirow{3}{*}{ 21.09 }  & & \\\cline{2-2}\cline{3-3}
Nov & \multirow{1}{*}{ 7.45 }  & \multirow{2}{*}{ 12.05 }  & & & \\\cline{2-2}
Dez & \multirow{1}{*}{ 4.59 }  & & & & \\\cline{2-2}\cline{3-3}\cline{4-4}\cline{5-5}\cline{6-6}
\hline\end{tabular}
\end{center}

==> tables/tabPCA1CPP.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c | c | c |}\cline{2-7}
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{PC1}          & \multicolumn{2}{c|}{PC2} & \multicolumn{2}{c|}{PC3}  \\\cline{2-7}\multicolumn{1}{c|}{} & $\mu$            & $\sigma$ & $\mu$         & $\sigma$ & $\mu$ & $\sigma$  \\\hline
$cc$ & 3.61  & 2.13  & 91.86  & 3.24  & 3.59  & 0.98 \\
$k$ & 48.24  & 0.99  & 2.96  & 2.25  & 48.25  & 0.43 \\
$bt$ & 48.15  & 1.14  & 5.18  & 3.89  & 48.16  & 0.56 \\\hline\hline
$\lambda$ & 65.24  & 0.51  & 33.30  & 0.17  & 1.46  & 0.49 \\
\hline\end{tabular}
\end{center}


==> tables/tabPCA1ExtraF.tex <==
$cc$ & 25.80  & 12.22  & 11.54  & 5.04  & 0.94  & 58.87  & 78.22  & 68.86  & 90.39  & 88.86  & 6.95  & 1.13  & 18.20  & 3.02  & 5.90 \\
$k$ & 36.43  & 43.96  & 45.61  & 47.40  & 49.50  & 25.66  & 9.98  & 6.10  & 7.63  & 6.42  & 44.94  & 49.52  & 42.00  & 48.41  & 47.02 \\
$bt$ & 37.77  & 43.82  & 42.85  & 47.56  & 49.56  & 15.46  & 11.80  & 25.04  & 1.98  & 4.72  & 48.11  & 49.35  & 39.80  & 48.57  & 47.08 \\\hline\hline
$\lambda$ & 53.15  & 53.06  & 46.26  & 55.36  & 63.80  & 28.69  & 32.57  & 34.27  & 33.25  & 33.57  & 18.16  & 14.37  & 19.47  & 11.38  & 2.63 \\


==> tables/tabPCA1ExtraI.tex <==
$cc$ & 14.43  & 17.12  & 11.54  & 0.69  & 13.26  & 2.17  & 2.72  & 74.78  & 70.72  & 79.30  & 96.63  & 76.59  & 95.75  & 94.69  & 1.58  & 4.09  & 2.46  & 1.71  & 0.57  & 2.03  & 2.20 \\
$k$ & 42.68  & 41.77  & 44.37  & 49.65  & 43.41  & 48.94  & 48.67  & 13.85  & 11.48  & 8.31  & 2.35  & 11.26  & 0.14  & 0.52  & 49.07  & 48.42  & 48.94  & 49.14  & 49.76  & 49.01  & 48.93 \\
$bt$ & 42.89  & 41.11  & 44.09  & 49.66  & 43.34  & 48.89  & 48.61  & 11.37  & 17.80  & 12.39  & 1.02  & 12.15  & 4.12  & 4.79  & 49.35  & 47.49  & 48.60  & 49.15  & 49.67  & 48.96  & 48.87 \\\hline\hline
$\lambda$ & 64.58  & 61.97  & 56.95  & 62.01  & 50.92  & 64.82  & 64.83  & 31.57  & 30.98  & 32.56  & 33.35  & 32.51  & 33.33  & 33.32  & 3.85  & 7.05  & 10.50  & 4.64  & 16.57  & 1.85  & 1.86 \\


==> tables/tabPCA1LAD.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c | c | c |}\cline{2-7}
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{PC1}          & \multicolumn{2}{c|}{PC2} & \multicolumn{2}{c|}{PC3}  \\\cline{2-7}\multicolumn{1}{c|}{} & $\mu$            & $\sigma$ & $\mu$         & $\sigma$ & $\mu$ & $\sigma$  \\\hline
$cc$ & 6.42  & 4.05  & 86.60  & 5.50  & 5.19  & 1.45 \\
$k$ & 46.98  & 1.86  & 2.95  & 1.65  & 47.61  & 0.57 \\
$bt$ & 46.59  & 2.18  & 10.45  & 4.72  & 47.20  & 0.90 \\\hline\hline
$\lambda$ & 64.96  & 0.71  & 33.08  & 0.41  & 1.96  & 0.52 \\
\hline\end{tabular}
\end{center}


==> tables/tabPCA1LAU.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c | c | c |}\cline{2-7}
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{PC1}          & \multicolumn{2}{c|}{PC2} & \multicolumn{2}{c|}{PC3}  \\\cline{2-7}\multicolumn{1}{c|}{} & $\mu$            & $\sigma$ & $\mu$         & $\sigma$ & $\mu$ & $\sigma$  \\\hline
$cc$ & 6.03  & 3.73  & 87.60  & 5.25  & 4.52  & 0.93 \\
$k$ & 47.13  & 1.76  & 3.01  & 1.98  & 47.90  & 0.38 \\
$bt$ & 46.84  & 1.97  & 9.39  & 4.31  & 47.58  & 0.57 \\\hline\hline
$\lambda$ & 64.99  & 0.60  & 33.08  & 0.41  & 1.93  & 0.36 \\
\hline\end{tabular}
\end{center}


==> tables/tabPCA1MET.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c | c | c |}\cline{2-7}
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{PC1}          & \multicolumn{2}{c|}{PC2} & \multicolumn{2}{c|}{PC3}  \\\cline{2-7}\multicolumn{1}{c|}{} & $\mu$            & $\sigma$ & $\mu$         & $\sigma$ & $\mu$ & $\sigma$  \\\hline
$cc$ & 5.82  & 3.76  & 87.26  & 5.12  & 4.93  & 1.19 \\
$k$ & 47.18  & 1.82  & 4.35  & 4.01  & 47.63  & 0.57 \\
$bt$ & 47.01  & 1.96  & 8.40  & 4.22  & 47.44  & 0.67 \\\hline\hline
$\lambda$ & 64.94  & 0.76  & 33.13  & 0.45  & 1.93  & 0.62 \\
\hline\end{tabular}
\end{center}


==> tables/tabPCA2CPP.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c | c | c |}\cline{2-7}
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{PC1}          & \multicolumn{2}{c|}{PC2} & \multicolumn{2}{c|}{PC3}  \\\cline{2-7}\multicolumn{1}{c|}{} & $\mu$            & $\sigma$ & $\mu$         & $\sigma$ & $\mu$ & $\sigma$  \\\hline
$cc$ & 0.84  & 0.61  & 80.59  & 6.89  & 2.30  & 2.19 \\\hline
$s$ & 14.28  & 0.07  & 0.97  & 1.03  & 15.89  & 1.15 \\
$s^{in}$ & 14.18  & 0.12  & 2.89  & 1.71  & 13.50  & 5.19 \\
$s^{out}$ & 14.07  & 0.23  & 2.83  & 1.63  & 18.80  & 4.94 \\
$k$ & 14.42  & 0.08  & 0.78  & 0.67  & 7.48  & 2.71 \\
$k^{in}$ & 14.29  & 0.10  & 2.36  & 1.41  & 7.21  & 4.49 \\
$k^{out}$ & 14.16  & 0.12  & 3.62  & 1.83  & 8.79  & 4.58 \\
$bt$ & 13.76  & 0.22  & 5.96  & 1.88  & 26.03  & 7.94 \\\hline\hline
$\lambda$ & 83.32  & 1.42  & 12.60  & 0.08  & 2.61  & 1.15 \\
\hline\end{tabular}
\end{center}


==> tables/tabPCA2Extra.tex <==
$cc$ & 2.79  & 4.34  & 2.57  & 0.82  & 1.29  & 0.66  & 0.76  & 28.44  & 9.46  & 3.29  & 21.95  & 6.95  & 29.82  & 30.04  & 32.24  & 60.89  & 80.24  & 43.85  & 3.81  & 33.84  & 33.54 \\\hline
$s$ & 15.28  & 15.84  & 16.46  & 16.01  & 16.70  & 15.49  & 15.47  & 3.78  & 4.95  & 2.90  & 3.26  & 17.78  & 1.95  & 2.05  & 1.95  & 0.34  & 0.87  & 4.84  & 11.15  & 0.52  & 0.43 \\
$s^{in}$ & 14.48  & 12.81  & 13.62  & 14.63  & 4.50  & 11.85  & 11.84  & 11.77  & 18.29  & 17.41  & 12.44  & 16.19  & 19.03  & 18.81  & 5.38  & 5.03  & 0.93  & 11.16  & 30.41  & 21.48  & 21.71 \\
$s^{out}$ & 12.13  & 12.12  & 12.59  & 12.91  & 19.02  & 13.87  & 13.85  & 17.19  & 16.79  & 20.12  & 18.81  & 8.90  & 13.42  & 13.43  & 19.35  & 7.90  & 3.11  & 11.38  & 14.58  & 12.91  & 12.92 \\
$k$ & 15.32  & 16.22  & 16.12  & 16.20  & 21.12  & 15.48  & 15.46  & 3.13  & 4.18  & 6.25  & 2.88  & 9.26  & 3.32  & 3.24  & 1.84  & 0.09  & 1.16  & 0.11  & 2.22  & 4.26  & 4.30 \\
$k^{in}$ & 14.49  & 13.56  & 12.90  & 15.34  & 7.29  & 12.99  & 12.98  & 10.45  & 16.50  & 19.68  & 11.13  & 20.75  & 17.89  & 17.86  & 8.78  & 4.07  & 1.26  & 6.07  & 15.41  & 14.67  & 14.65 \\
$k^{out}$ & 11.70  & 11.25  & 11.80  & 9.24  & 21.09  & 14.20  & 14.19  & 19.14  & 20.50  & 21.19  & 26.13  & 0.19  & 12.36  & 12.28  & 18.80  & 7.50  & 4.68  & 20.44  & 10.57  & 12.14  & 12.20 \\
$bt$ & 13.82  & 13.86  & 13.93  & 14.86  & 8.99  & 15.47  & 15.45  & 6.10  & 9.32  & 9.16  & 3.41  & 19.99  & 2.20  & 2.29  & 11.66  & 14.20  & 7.75  & 2.17  & 11.86  & 0.18  & 0.25 \\\hline\hline
$\lambda$ & 71.73  & 60.58  & 60.35  & 64.53  & 41.28  & 70.06  & 70.08  & 15.23  & 21.53  & 20.13  & 16.42  & 22.83  & 13.83  & 13.86  & 9.95  & 11.37  & 12.25  & 11.19  & 15.71  & 11.43  & 11.38 \\


==> tables/tabPCA2LAD.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c | c | c |}\cline{2-7}
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{PC1}          & \multicolumn{2}{c|}{PC2} & \multicolumn{2}{c|}{PC3}  \\\cline{2-7}\multicolumn{1}{c|}{} & $\mu$            & $\sigma$ & $\mu$         & $\sigma$ & $\mu$ & $\sigma$  \\\hline
$cc$ & 1.83  & 1.11  & 80.38  & 11.45  & 3.78  & 4.43 \\\hline
$s$ & 14.25  & 0.17  & 1.34  & 1.81  & 9.88  & 5.76 \\
$s^{in}$ & 13.99  & 0.19  & 2.06  & 1.70  & 17.62  & 6.15 \\
$s^{out}$ & 14.03  & 0.22  & 1.81  & 1.98  & 15.44  & 6.68 \\
$k$ & 14.38  & 0.13  & 0.95  & 1.64  & 3.45  & 3.15 \\
$k^{in}$ & 14.05  & 0.14  & 2.26  & 1.66  & 13.44  & 7.26 \\
$k^{out}$ & 13.96  & 0.15  & 1.72  & 1.53  & 16.14  & 6.37 \\
$bt$ & 13.51  & 0.35  & 9.48  & 2.86  & 20.26  & 9.87 \\\hline\hline
$\lambda$ & 82.32  & 1.61  & 12.52  & 0.26  & 2.97  & 1.21 \\
\hline\end{tabular}
\end{center}


==> tables/tabPCA2LAU.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c | c | c |}\cline{2-7}
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{PC1}          & \multicolumn{2}{c|}{PC2} & \multicolumn{2}{c|}{PC3}  \\\cline{2-7}\multicolumn{1}{c|}{} & $\mu$            & $\sigma$ & $\mu$         & $\sigma$ & $\mu$ & $\sigma$  \\\hline
$cc$ & 1.59  & 0.81  & 80.37  & 5.18  & 3.09  & 1.89 \\\hline
$s$ & 14.40  & 0.15  & 0.81  & 0.68  & 4.75  & 4.43 \\
$s^{in}$ & 14.00  & 0.14  & 2.32  & 1.49  & 18.98  & 4.93 \\
$s^{out}$ & 13.96  & 0.14  & 2.72  & 1.44  & 18.25  & 6.36 \\
$k$ & 14.49  & 0.15  & 0.54  & 0.35  & 1.37  & 0.98 \\
$k^{in}$ & 14.01  & 0.13  & 2.72  & 1.35  & 18.69  & 5.01 \\
$k^{out}$ & 13.85  & 0.13  & 2.37  & 1.73  & 22.63  & 3.79 \\
$bt$ & 13.69  & 0.22  & 8.16  & 1.62  & 12.23  & 8.33 \\\hline\hline
$\lambda$ & 81.87  & 0.88  & 12.48  & 0.15  & 3.33  & 0.70 \\
\hline\end{tabular}
\end{center}


==> tables/tabPCA2MET.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c | c | c |}\cline{2-7}
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{PC1}          & \multicolumn{2}{c|}{PC2} & \multicolumn{2}{c|}{PC3}  \\\cline{2-7}\multicolumn{1}{c|}{} & $\mu$            & $\sigma$ & $\mu$         & $\sigma$ & $\mu$ & $\sigma$  \\\hline
$cc$ & 1.16  & 0.76  & 81.72  & 3.00  & 1.61  & 1.78 \\\hline
$s$ & 14.32  & 0.16  & 1.76  & 1.12  & 11.39  & 5.50 \\
$s^{in}$ & 14.17  & 0.11  & 2.29  & 1.29  & 14.46  & 3.72 \\
$s^{out}$ & 14.09  & 0.17  & 1.72  & 1.18  & 17.54  & 5.37 \\
$k$ & 14.39  & 0.16  & 1.73  & 0.63  & 4.76  & 2.82 \\
$k^{in}$ & 14.12  & 0.13  & 1.02  & 0.71  & 11.69  & 6.93 \\
$k^{out}$ & 14.06  & 0.13  & 3.11  & 1.58  & 12.18  & 9.24 \\
$bt$ & 13.69  & 0.26  & 6.64  & 2.01  & 26.37  & 12.37 \\\hline\hline
$\lambda$ & 83.41  & 1.53  & 12.53  & 0.11  & 2.34  & 1.16 \\
\hline\end{tabular}
\end{center}


==> tables/tabPCA3Extra.tex <==
$cc$ & 3.46  & 4.19  & 2.44  & 0.36  & 2.18  & 1.28  & 1.17  & 3.06  & 1.61  & 1.23  & 1.19  & 2.57  & 3.03  & 2.17  & 17.36  & 16.88  & 21.68  & 17.00  & 10.00  & 18.65  & 19.13 \\\hline
$s$ & 10.05  & 9.21  & 9.60  & 9.31  & 3.54  & 10.27  & 10.59  & 5.81  & 5.74  & 7.33  & 8.47  & 9.24  & 6.26  & 5.96  & 4.58  & 8.02  & 4.91  & 2.21  & 13.10  & 0.92  & 1.53 \\
$s^{in}$ & 9.57  & 8.03  & 9.21  & 8.74  & 0.78  & 7.75  & 7.99  & 4.63  & 0.59  & 1.27  & 6.69  & 2.77  & 5.38  & 5.29  & 8.22  & 12.82  & 9.18  & 6.53  & 7.63  & 5.90  & 4.77 \\
$s^{out}$ & 7.88  & 6.21  & 5.45  & 6.97  & 5.76  & 9.25  & 9.54  & 6.78  & 10.23  & 12.76  & 9.20  & 10.26  & 5.27  & 4.92  & 5.90  & 2.99  & 3.86  & 8.43  & 10.84  & 4.58  & 4.76 \\
$k$ & 10.44  & 10.02  & 9.88  & 10.39  & 5.80  & 10.80  & 11.05  & 4.62  & 5.13  & 5.66  & 5.54  & 14.08  & 4.48  & 4.29  & 3.63  & 6.02  & 6.18  & 1.86  & 1.21  & 1.33  & 1.30 \\
$k^{in}$ & 10.12  & 9.30  & 9.50  & 9.98  & 4.43  & 8.64  & 8.86  & 2.69  & 0.70  & 0.88  & 4.49  & 9.61  & 5.40  & 5.50  & 7.12  & 10.55  & 8.70  & 6.17  & 8.24  & 7.27  & 6.54 \\
$k^{out}$ & 7.27  & 5.29  & 4.43  & 5.43  & 9.11  & 10.10  & 10.33  & 8.36  & 12.52  & 13.63  & 5.65  & 11.61  & 3.38  & 3.08  & 7.82  & 5.77  & 2.07  & 13.52  & 5.68  & 5.00  & 4.65 \\
$bt$ & 9.62  & 7.97  & 7.53  & 8.93  & 2.25  & 10.47  & 10.78  & 3.77  & 8.42  & 9.14  & 6.95  & 8.12  & 5.60  & 5.29  & 2.72  & 0.42  & 1.99  & 2.74  & 8.66  & 1.16  & 1.60 \\\hline
$asy$ & 5.42  & 7.05  & 7.97  & 8.48  & 15.47  & 6.16  & 5.79  & 14.17  & 12.88  & 11.78  & 11.02  & 4.67  & 12.48  & 13.39  & 2.95  & 1.03  & 0.58  & 2.71  & 0.87  & 6.54  & 5.80 \\
$\mu^{asy}$ & 5.48  & 6.99  & 7.99  & 8.47  & 15.44  & 6.18  & 5.80  & 14.12  & 13.04  & 11.78  & 11.01  & 4.72  & 12.46  & 13.37  & 2.92  & 0.76  & 0.75  & 2.77  & 0.76  & 6.58  & 5.83 \\
$\sigma^{asy}$ & 6.53  & 7.39  & 7.63  & 7.15  & 2.37  & 5.59  & 5.48  & 1.69  & 3.80  & 1.75  & 8.46  & 7.49  & 5.94  & 5.45  & 11.32  & 8.91  & 11.14  & 3.04  & 15.54  & 13.70  & 15.31 \\
$dis$ & 5.02  & 6.67  & 7.78  & 8.08  & 15.41  & 5.98  & 5.59  & 14.12  & 13.41  & 11.92  & 11.53  & 4.80  & 12.45  & 13.38  & 4.99  & 1.40  & 0.67  & 3.02  & 0.83  & 7.44  & 6.69 \\
$\mu^{dis}$ & 5.33  & 7.01  & 7.24  & 6.92  & 14.34  & 5.49  & 5.14  & 13.33  & 10.15  & 9.47  & 8.02  & 5.05  & 11.86  & 12.65  & 1.66  & 7.08  & 5.72  & 11.38  & 2.68  & 0.77  & 0.66 \\
$\sigma^{dis}$ & 3.82  & 4.68  & 3.34  & 0.81  & 3.12  & 2.03  & 1.88  & 2.85  & 1.77  & 1.39  & 1.77  & 5.00  & 6.01  & 5.24  & 18.82  & 17.36  & 22.58  & 18.61  & 13.97  & 20.16  & 21.42 \\\hline\hline
$\lambda$ & 46.11  & 43.48  & 44.29  & 46.95  & 30.34  & 44.12  & 43.52  & 26.42  & 24.97  & 24.76  & 19.99  & 23.91  & 25.98  & 26.13  & 14.90  & 14.72  & 11.82  & 13.16  & 17.32  & 11.62  & 12.15 \\


==> tables/tabPCA3LAD.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c | c | c |}\cline{2-7}
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{PC1}          & \multicolumn{2}{c|}{PC2} & \multicolumn{2}{c|}{PC3}  \\\cline{2-7}\multicolumn{1}{c|}{} & $\mu$            & $\sigma$ & $\mu$         & $\sigma$ & $\mu$ & $\sigma$  \\\hline
$cc$ & 1.96  & 0.95  & 3.07  & 1.46  & 17.94  & 5.38 \\\hline
$s$ & 12.34  & 0.57  & 1.72  & 0.99  & 2.43  & 0.93 \\
$s^{in}$ & 12.06  & 0.64  & 3.18  & 0.98  & 1.98  & 1.09 \\
$s^{out}$ & 12.22  & 0.48  & 1.14  & 0.78  & 2.83  & 0.79 \\
$k$ & 12.54  & 0.56  & 1.43  & 0.87  & 0.92  & 0.44 \\
$k^{in}$ & 12.15  & 0.61  & 3.81  & 0.79  & 0.61  & 0.42 \\
$k^{out}$ & 12.27  & 0.45  & 1.51  & 1.08  & 1.56  & 0.39 \\
$bt$ & 11.73  & 0.64  & 1.80  & 0.88  & 2.28  & 1.00 \\\hline
$asy$ & 1.51  & 0.97  & 19.66  & 1.63  & 3.02  & 1.66 \\
$\mu^{asy}$ & 1.41  & 0.99  & 19.53  & 1.62  & 3.00  & 1.69 \\
$\sigma^{asy}$ & 5.62  & 0.68  & 2.01  & 1.23  & 27.46  & 3.31 \\
$dis$ & 1.58  & 0.98  & 19.57  & 1.65  & 3.21  & 1.71 \\
$\mu^{dis}$ & 1.84  & 1.00  & 18.62  & 1.52  & 2.08  & 1.13 \\
$\sigma^{dis}$ & 0.77  & 0.59  & 2.94  & 1.60  & 30.68  & 3.34 \\\hline\hline
$\lambda$ & 48.65  & 1.03  & 27.84  & 0.31  & 13.00  & 0.77 \\
\hline\end{tabular}
\end{center}


==> tables/tabPCA3LAU.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c | c | c |}\cline{2-7}
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{PC1}          & \multicolumn{2}{c|}{PC2} & \multicolumn{2}{c|}{PC3}  \\\cline{2-7}\multicolumn{1}{c|}{} & $\mu$            & $\sigma$ & $\mu$         & $\sigma$ & $\mu$ & $\sigma$  \\\hline
$cc$ & 1.64  & 0.77  & 2.42  & 1.71  & 19.20  & 3.96 \\\hline
$s$ & 12.80  & 0.46  & 0.89  & 0.82  & 2.53  & 0.63 \\
$s^{in}$ & 12.47  & 0.42  & 2.30  & 0.97  & 2.29  & 0.81 \\
$s^{out}$ & 12.37  & 0.46  & 2.89  & 1.24  & 2.64  & 0.58 \\
$k$ & 12.93  & 0.44  & 0.82  & 0.73  & 1.32  & 0.45 \\
$k^{in}$ & 12.54  & 0.37  & 2.88  & 1.13  & 1.02  & 0.56 \\
$k^{out}$ & 12.32  & 0.46  & 3.82  & 1.14  & 1.57  & 0.68 \\
$bt$ & 12.19  & 0.46  & 1.06  & 0.62  & 2.64  & 0.89 \\\hline
$asy$ & 0.93  & 0.81  & 20.38  & 0.82  & 1.66  & 1.09 \\
$\mu^{asy}$ & 0.96  & 0.83  & 20.26  & 0.82  & 1.66  & 1.04 \\
$\sigma^{asy}$ & 6.18  & 0.71  & 1.24  & 0.92  & 27.98  & 1.74 \\
$dis$ & 0.90  & 0.79  & 20.36  & 0.82  & 1.54  & 1.07 \\
$\mu^{dis}$ & 0.92  & 0.61  & 19.02  & 0.84  & 1.45  & 1.12 \\
$\sigma^{dis}$ & 0.86  & 0.51  & 1.64  & 1.10  & 32.51  & 1.90 \\\hline\hline
$\lambda$ & 48.41  & 0.52  & 27.95  & 0.36  & 12.81  & 0.79 \\
\hline\end{tabular}
\end{center}


==> tables/tabPCA3MET.tex <==
\begin{center}
\begin{tabular}{| l || c | c | c | c | c | c |}\cline{2-7}
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{PC1}          & \multicolumn{2}{c|}{PC2} & \multicolumn{2}{c|}{PC3}  \\\cline{2-7}\multicolumn{1}{c|}{} & $\mu$            & $\sigma$ & $\mu$         & $\sigma$ & $\mu$ & $\sigma$  \\\hline
$cc$ & 1.18  & 0.71  & 3.00  & 2.35  & 22.39  & 2.71 \\\hline
$s$ & 12.34  & 0.66  & 1.74  & 1.17  & 1.55  & 0.75 \\
$s^{in}$ & 12.25  & 0.62  & 1.74  & 0.96  & 1.45  & 0.77 \\
$s^{out}$ & 12.11  & 0.72  & 2.42  & 1.35  & 1.78  & 0.78 \\
$k$ & 12.48  & 0.63  & 1.46  & 0.91  & 0.54  & 0.48 \\
$k^{in}$ & 12.32  & 0.56  & 1.54  & 1.22  & 0.65  & 0.62 \\
$k^{out}$ & 12.12  & 0.67  & 3.10  & 1.15  & 0.87  & 0.74 \\
$bt$ & 11.85  & 0.62  & 1.46  & 0.87  & 1.16  & 0.70 \\\hline
$asy$ & 1.79  & 1.22  & 19.35  & 2.15  & 3.29  & 2.15 \\
$\mu^{asy}$ & 1.84  & 1.22  & 19.17  & 2.16  & 3.31  & 2.23 \\
$\sigma^{asy}$ & 4.17  & 0.79  & 3.91  & 2.35  & 27.79  & 3.96 \\
$dis$ & 1.78  & 1.18  & 19.26  & 2.15  & 3.38  & 2.29 \\
$\mu^{dis}$ & 1.53  & 1.10  & 18.23  & 2.12  & 3.32  & 1.71 \\
$\sigma^{dis}$ & 2.23  & 0.93  & 3.61  & 2.38  & 28.54  & 3.23 \\\hline\hline
$\lambda$ & 49.05  & 1.01  & 27.79  & 0.30  & 13.30  & 1.35 \\
\hline\end{tabular}
\end{center}


==> tables/tabSectorsExtra.tex <==
F1 & 53.11  & 43.31  & 3.58 \\\hline
F2 & 58.98  & 39.29  & 1.72 \\\hline
F3 & 65.41  & 31.87  & 2.72 \\\hline
F4 & 66.49  & 32.03  & 1.48 \\\hline
F5 & 62.98  & 36.12  & 0.90 \\\hline
I1 & 4.81  & 94.23  & 0.96 \\\hline
I2 & 53.12  & 45.31  & 1.56 \\\hline
I3 & 58.41  & 40.19  & 1.40 \\\hline
I4 & 39.06  & 59.43  & 1.51 \\\hline
I5 & 54.95  & 43.69  & 1.35 \\\hline
TT1 & 74.86  & 24.49  & 0.65 \\\hline
TT2 & 76.57  & 22.86  & 0.57 \\\hline

